Your LR Schedule May Not Be Principled: Effective Learning Rate Scheduling in Weight-Normalized Training

Weight-normalized (WN) training is emerging as a compelling alternative to conventional weight decay (WD), with recent studies reporting substantial pretraining loss gains. We find that the effective learning rate (ELR) trajectory accounts for most of the loss dynamics difference between WN and WD. Matching blockwise ELR trajectories step by step closely aligns their loss curves. Schedule design should therefore target ELR rather than the nominal learning rate (LR). Building on this principle, we model directional-alignment dynamics under WN and derive $1/\sqrt{t}$ decay as the optimal schedule. For finite-horizon pretraining, we propose AIR (Affine Inverse-square-Root decay) to match prescribed peak and terminal LRs. Experiments on 128B- and 500B-token Mixture-of-Experts pretraining under WN show that AIR outperforms cosine and alternative schedules in loss, downstream performance, and hyperparameter robustness, reducing terminal training loss by 0.01 relative to cosine. We further identify late-stage scheduling as the primary source of this gain through controlled stage interventions, and demonstrate that a shared late schedule progressively attenuates alignment differences left by earlier LRs. Finally, transferring AIR's ELR trajectory to WD reproduces the same improved loss dynamics, demonstrating that these gains come from ELR scheduling itself and extend beyond fixed-norm training.

==> common.tex <==
% Shared paper-facing commands for both ICLR (`main.tex`) and Seed
% (`seed_main.tex`) entries. Keep math macros in `math_commands.tex`.
% Pattern follows icml2026_PL_Width/common.tex.

\RequirePackage{graphicx}
\RequirePackage{xcolor}
\RequirePackage{xspace}
\RequirePackage{CJKutf8} % Draft only: remove with Chinese notes before submission.
\RequirePackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\setlength{\marginparwidth}{1.5cm}
\newcommand{\zh}[1]{\begin{CJK*}{UTF8}{gbsn}#1\end{CJK*}}
\newcommand{\qifantodo}[1]{\todo[author=Qifan]{\zh{#1}}}
\newcommand{\xinyutodo}[1]{\todo[author=Xinyu]{\zh{#1}}}
\newcommand{\xingyantodo}[1]{\todo[author=Xingyan]{\zh{#1}}}
\newcommand{\dihetodo}[1]{\todo[author=Di He]{\zh{#1}}}

% Paper-facing title. `\mytitle` is the display form (line breaks);
% `\mytitleplain` is the one-line PDF metadata / hypersetup form.
\newcommand{\mytitleplain}{Your LR Schedule May Not Be Principled: Effective Learning Rate Scheduling in Weight-Normalized Training}
\newcommand{\mytitle}{Your LR Schedule May Not Be Principled:\\Effective Learning Rate Scheduling in\\Weight-Normalized Training}

% Paper-facing scheduler name. Edit this block together if the public name
% changes. Running text uses \OurMethod (short name). First mention writes
% \OurMethod (\OurMethodDef). Math uses \OurMethodMath.
% \OurMethodDef is the full name only, not a bundled ``short (full)'' form.
% Running-text macros use \xspace so `\OurMethod against` keeps the following
% space; do not write `\OurMethod{}` as well, or a double space can appear.
\newcommand{\OurMethodShort}{AIR}
\newcommand{\OurMethodDef}{\textbf{A}ffine \textbf{I}nverse-square-\textbf{R}oot decay\xspace}
\newcommand{\OurMethod}{\OurMethodShort\xspace}
\newcommand{\OurMethodMath}{\mathrm{\OurMethodShort}}

% Possessive narrative citation: "D'Angelo et al.'s (2024)" in ICLR authoryear
% and "D'Angelo et al.'s [N]" in Seed numerical natbib.
\makeatletter
\newcommand{\citeposs}[1]{\citeauthor{#1}'s~\ifNAT@numbers\citep{#1}\else\citeyearpar{#1}\fi}
\makeatother

